Multi-intent-aware Session-based Recommendation

Session-based recommendation (SBR) aims to predict the following item a user will interact with during an ongoing session. Most existing SBR models focus on designing sophisticated neural-based encoders to learn a session representation, capturing the relationship among session items. However, they tend to focus on the last item, neglecting diverse user intents that may exist within a session. This limitation leads to significant performance drops, especially for longer sessions. To address this issue, we propose a novel SBR model, called Multi-intent-aware Session-based Recommendation Model (MiaSRec). It adopts frequency embedding vectors indicating the item frequency in session to enhance the information about repeated items. MiaSRec represents various user intents by deriving multiple session representations centered on each item and dynamically selecting the important ones. Extensive experimental results show that MiaSRec outperforms existing state-of-the-art SBR models on six datasets, particularly those with longer average session length, achieving up to 6.27% and 24.56% gains for MRR@20 and Recall@20. Our code is available at https://github.com/jin530/MiaSRec.

==> Figures_tex/Fig_alpha.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.22\textwidth]{Figures/DIGI_alpha.png} &
\includegraphics[width=0.22\textwidth]{Figures/RR_alpha.png} \\
(a) Diginetica & (b) Retailrocket \\
\end{tabular}
\caption{R@20 of EDISON for varying the ${\alpha}$ of transformation function ${\alpha}$-entmax. The larger the ${\alpha}$, the higher the sparsity, and therefore the fewer interests are extracted.}
\label{fig:exp_alpha}
\end{figure}
% , and when $\mathbf{\beta}$=$0$ equals to softmax, so the number of interests $k$ is equal to the number of session items $|s|$

==> Figures_tex/Fig_beta.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.22\textwidth]{Figures/DIGI_beta.png} &
\includegraphics[width=0.22\textwidth]{Figures/RR_beta.png} \\
(a) Diginetica & (b) Retailrocket \\
\end{tabular}
\caption{R@20 of EDISON for varying the combination hyperparameter ${\beta}$.}
\label{fig:exp_beta}
\end{figure}
% ${\beta}$=$0$ and ${\beta}$=$1$ equal solely utilizing average-pooling and max-pooling, respectively.

==> Figures_tex/Fig_hyperparameter.tex <==
\begin{figure*}[t]
\centering
\begin{tabular}{ccc}
\includegraphics[width=0.3\textwidth]{Figures/DIGI_temperature.png} &
\includegraphics[width=0.3\textwidth]{Figures/DIGI_dropoutSI.png} &
\includegraphics[width=0.3\textwidth]{Figures/DIGI_dropoutT.png} \\
\end{tabular} \\
(a) Diginetica \\

\begin{tabular}{ccc}
\includegraphics[width=0.3\textwidth]{Figures/RR_temperature.png} &
\includegraphics[width=0.3\textwidth]{Figures/RR_dropoutSI.png} &
\includegraphics[width=0.3\textwidth]{Figures/RR_dropoutT.png} \\
\end{tabular} \\
(b) Retailrocket  \\

\begin{tabular}{ccc}
\includegraphics[width=0.3\textwidth]{Figures/YC_temperature.png} &
\includegraphics[width=0.3\textwidth]{Figures/YC_dropoutSI.png}  &
\includegraphics[width=0.3\textwidth]{Figures/YC_dropoutT.png} \\
\end{tabular} \\
(c) Yoochoose \\

\caption{Accuracy of EDISON over varying the hyperparameters: temperature $\tau$, embedding dropout ratio $\delta_{emb}$, and transformer layer dropout ratio $\delta_{tr}$.}
\label{fig:exp_hyperparameter}
\end{figure*}

% \includegraphics[width=1.0\linewidth]{Figures/empty.png}
% \caption{Parameter tuning of EDISON.}\label{fig:hyperparameter}
% \vskip -0.1in
% \end{figure}



==> Figures_tex/Fig_k_representation.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{c}
\includegraphics[width=0.33\textwidth]{Figures/K_Legend.png} \\
\end{tabular}
\begin{tabular}{cc}
\includegraphics[width=0.22\textwidth]{Figures/DIGI_K_v3.png} &
\includegraphics[width=0.22\textwidth]{Figures/RR_K_v3.png} \\
 &  \\
% (a) Retailrocket & (b) Diginetica \\
\end{tabular}

\begin{tabular}{c}
\includegraphics[width=0.25\textwidth]{Figures/K_Legend_multi_v2.png} \\
\end{tabular}
\begin{tabular}{cc}
\includegraphics[width=0.22\textwidth]{Figures/DIGI_K_multi_v3.png} &
\includegraphics[width=0.22\textwidth]{Figures/RR_K_multi_v3.png} \\
(a) Diginetica & (b) Retailrocket \\
\end{tabular}
\caption{R@20 of EDISON and other competing models for varying the number of session vectors $k$. EDISON extracts top-$k$ contextualized item vectors for session vectors. Meanwhile, ComiRec and Re4 always utilize $k$ session vectors.}
\label{fig:exp_last_k}
\end{figure}

% When $k$ is 50 (\ie, the max sequence length), EDISON extracts all item vectors for each session.
% competing multi-interest models for varying the number of session vectors $k$. For each session, due to the way modeling multi-interest, EDISON utilizes $\min (k, |s|+1)$ session vectors, whereas the other models always utilize $k$ session vectors.

==> Figures_tex/Fig_oracle_analysis.tex <==
% \begin{figure}[t]
% \centering
% \begin{tabular}{cc}
% \includegraphics[width=0.215\textwidth]{Figures/DIGI_oracle_v3.png} &
% \includegraphics[width=0.215\textwidth]{Figures/RR_oracle_v3.png}  \\
% % \includegraphics[width=0.28\textwidth]{Figures/YC_oracle_v3.png} \\
% (a) Diginetica & (b) Retailrocket \\
% % \includegraphics[width=0.28\textwidth]{Figures/Tmall_oracle.png} &
% % \includegraphics[width=0.28\textwidth]{Figures/Dressipi_oracle.png}  & 
% % \includegraphics[width=0.28\textwidth]{Figures/LastFM_oracle.png} \\
% % (d) Tmall & (e) Dressipi & (f) LastFM\\

% \end{tabular}
% \caption{Distribution of user interests for long sessions using the optimal session extractor. The interest position indicates how far the user interest is from the last item (the last item is position 1).}\label{fig:exp_oracle_analysis}
% \end{figure}


\begin{figure*}[t]
\centering
\begin{tabular}{ccc}
\includegraphics[width=0.26\textwidth]{Figures/DIGI_oracle_v3.png} &
\includegraphics[width=0.26\textwidth]{Figures/RR_oracle_v3.png}  & 
\includegraphics[width=0.26\textwidth]{Figures/YC_oracle_v3.png} \\
(a) Diginetica & (b) Retailrocket & (c) Yoochoose \\
\includegraphics[width=0.26\textwidth]{Figures/Tmall_oracle_v2.png} &
\includegraphics[width=0.26\textwidth]{Figures/Dressipi_oracle_v2.png}  & 
\includegraphics[width=0.26\textwidth]{Figures/LastFM_oracle_v2.png} \\
(d) Tmall & (e) Dressipi & (f) LastFM \\

\end{tabular}
\caption{Distribution of user interests for long sessions using the optimal extractor. The interest position indicates how far the user interest is from the last item (the last item is position 1).}\label{fig:exp_oracle_analysis}
\end{figure*}

% \includegraphics[width=1.0\linewidth]{Figures/empty.png}
% \caption{Parameter tuning of EDISON.}\label{fig:hyperparameter}
% \vskip -0.1in
% \end{figure}



==> Figures_tex/Fig_session_length_2column.tex <==
% \begin{figure}[t]
% \centering
% \begin{tabular}{c}
% \includegraphics[width=0.45\textwidth]{Figures/Legend_length_v3.png} \\
% \end{tabular}
% \begin{tabular}{cc}
% \includegraphics[width=0.215\textwidth]{Figures/DIGI_length_v4.png}  &
% \includegraphics[width=0.215\textwidth]{Figures/RR_length_v4.png} \\
% % \includegraphics[width=0.26\textwidth]{Figures/YC_length_v4.png} \\
% (a) Diginetica & (b) Retailrocket \\
% % (a) Diginetica & (b) Retailrocket & (c) Yoochoose\\
% \end{tabular}
% \caption{Performance (R@20) of SBR models over varying session lengths. Sessions are divided into six groups based on session length. CORE~\cite{hou2022core}, NISER+~\cite{GuptaGMVS19NISER}, and SASRec~\cite{KangM18SASRec} are single session representation models and Re4~\cite{ZhangYYLFZC022Re4}, ComiRec~\cite{ChenZZXX21ComiRec}, and EDISON are multiple session representation models.}\label{fig:exp_session_length}
% \vspace{-3mm}
% \end{figure}



\begin{figure*}[t]
\centering
\begin{tabular}{c}
\includegraphics[width=0.5\textwidth]{Figures/Legend_length_v4.png} \\
\end{tabular}
\begin{tabular}{ccc}
\includegraphics[width=0.26\textwidth]{Figures/DIGI_length_v4.png}  &
\includegraphics[width=0.26\textwidth]{Figures/RR_length_v4.png} &
\includegraphics[width=0.26\textwidth]{Figures/YC_length_v4.png} \\
% \includegraphics[width=0.3\textwidth]{Figures/DIGI_length_gain_v2.png}  &
% \includegraphics[width=0.3\textwidth]{Figures/RR_length_gain_v2.png} &
% \includegraphics[width=0.3\textwidth]{Figures/YC_length_gain_v2.png} \\
(a) Diginetica & (b) Retailrocket & (c) Yoochoose\\
\end{tabular}
\caption{Performance (R@20) of SBR models over varying session lengths. Sessions are divided into six groups based on session length. CORE~\cite{hou2022core}, NISER+~\cite{GuptaGMVS19NISER}, and SASRec~\cite{KangM18SASRec} are single session representation models, and ComiRec~\cite{ChenZZXX21ComiRec}, Re4~\cite{ZhangYYLFZC022Re4}, and EDISON are multiple session representation models.
}\label{fig:exp_session_length}
\vspace{-3mm}
\end{figure*}

% and relative improvement ratios over SASRec~\cite{KangM18SASRec} 
% For too short ($\le$ 5) or too long ($\ge$ 15) sessions, we report the average accuracy.

==> Tables/tab_backbone.tex <==
\begin{table}[]\small
\centering
\begin{tabular}{c|cc|cc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c|}{Diginetica} & \multicolumn{2}{c}{Retailrocket} \\
                                  & R@20           & M@20         & R@20            & M@20          \\ 
\midrule
EDISON                            & \textbf{53.32}          & \textbf{19.32}          & \textbf{62.92}           & \textbf{39.50}           \\
EDISON$_{\text{Last}}$            & 51.98          & 18.25          & 61.56           & 37.75           \\
\midrule
SASRec$_{\text{Multi}}$           & 50.78          & 17.68          & 61.00           & 36.65           \\ 
SASRec                            & 49.86          & 17.20          & 59.70           & 35.71           \\
\midrule
NISER+$_{\text{Multi}}$           & 51.54          &18.71          & 61.17           & 38.82           \\
NISER+                            & 51.11          & 18.21          & 60.70           & 38.18           \\
 \bottomrule
\end{tabular}
\caption{Effect of multiple session representation for various backbone models. EDISON$_{\text{Last}}$ only uses the last item vector. SASRec$_{\text{Multi}}$ and NISER+$_{\text{Multi}}$, utilize multiple representations using the same extractor and aggregator of EDISON. }\label{tab:exp_backbone}
\end{table}



==> Tables/tab_cutoff5_overall_performance.tex <==
\begin{table*} \small
\centering
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{c|c|cccccc|cccc|c|r}
\toprule
Dataset & Metric & SASRec & SR-GNN & NISER+ & SGNN-HN & DSAN & CORE & SINE & A-mixer & ComiRec & Re4 & EDISON & \multicolumn{1}{c}{Imp.} \\ \midrule
\multirow{2}{*}{Diginetica} & R@5 & 25.73 & 25.01 & 27.48 & 26.46 & 27.88 & \ul{ 28.51} & 24.07 & 25.01 & 27.62 & 27.91 & \textbf{29.30$^{\ddagger}$} & 2.77\% \\
 & M@5 & 14.84 & 14.33 & 15.87 & 14.89 & 15.85 & 16.12 & 13.91 & 14.30 & 16.02 & \ul{ 16.14} & \textbf{16.92$^{\dagger}$} & 4.88\% \\ \midrule
\multirow{2}{*}{Retailrocket} & R@5 & 45.03 & 45.88 & 48.13 & 45.11 & \ul{ 48.45} & 48.12 & 42.50 & 45.42 & 48.35 & 48.39 & \textbf{49.94$^{\ddagger}$} & 3.08\% \\
 & M@5 & 34.21 & 34.75 & 36.89 & 34.12 & \ul{ 37.37} & 37.09 & 32.87 & 34.87 & 36.80 & 36.74 & \textbf{38.00$^{\ddagger}$} & 1.69\% \\ \midrule
\multirow{2}{*}{Yoochoose} & R@5 & 43.41 & 42.86 & 43.46 & 41.65 & 43.75 & \ul{ 44.10} & 37.69 & 42.37 & 42.44 & 43.05 & \textbf{44.31} & 0.48\% \\
 & M@5 & 26.51 & 26.31 & 26.94 & 25.86 & \ul{ 27.11} & 26.08 & 23.00 & 25.86 & 25.91 & 26.17 & \textbf{27.52} & 1.51\% \\ \midrule
\multirow{2}{*}{Tmall} & R@5 & 29.21 & 28.56 & 34.59 & 30.82 & 36.70 & \ul{ 37.86} & 27.64 & 33.79 & 34.05 & 34.54 & \textbf{43.25$^{\ddagger}$} & 14.25\% \\
 & M@5 & 24.41 & 24.25 & 28.88 & 23.25 & 30.22 & \ul{ 30.85} & 26.69 & 27.76 & 27.18 & 27.62 & \textbf{32.37$^{\ddagger}$} & 4.90\% \\ \midrule
\multirow{2}{*}{Dressipi} & R@5 & 21.21 & 21.55 & 22.91 & 22.84 & 22.46 & 23.24 & 23.11 & 20.72 & \ul{ 24.38} & 24.12 & \textbf{25.10$^{\dagger}$} & 2.95\% \\
 & M@5 & 12.72 & 13.05 & 13.81 & 13.49 & 13.60 & 14.04 & 13.95 & 12.34 & \ul{ 14.53} & 14.40 & \textbf{14.67$^{\dagger}$} & 0.99\% \\ \midrule
\multirow{2}{*}{LastFM} & R@5 & 9.56 & 11.78 & 12.01 & 11.38 & 11.45 & 11.64 & 11.19 & 10.62 & 11.52 & \ul{ 12.38} & \textbf{13.73$^{\ddagger}$} & 10.85\% \\
 & M@5 & 5.17 & 7.74 & \ul{ 7.79} & 6.57 & 6.87 & 6.77 & 6.52 & 6.49 & 6.81 & 7.47 & \textbf{8.18$^{\dagger}$} & 5.05\% \\
\bottomrule
\end{tabular}
\caption{Performance comparison for the proposed method and baseline models. Imp. indicates how much better EDISON is than the best baseline model. The best model is marked bold and the second best model is underlined. Significant differences ($\rho < 0.05$ and $\rho < 0.01$) between the best baseline model and EDISON are reported with $\dagger$ and $\ddagger$.}\label{tab:exp_all_cutoff5}
\end{table*}

==> Tables/tab_framework.tex <==
\begin{table}[] \small
\begin{tabular}{c|c|c}
\toprule
Model & \begin{tabular}[c]{@{}c@{}}Multiple\\ session vectors\end{tabular} & Aggregator \\ \midrule
\begin{tabular}[c]{@{}c@{}}
GRU4Rec, NARM, \\ 
SASRec, SR-GNN, \\ 
NISER+, SGNN-HN,\\ 
LESSR, CL4SRec, \\ 
CORE, Atten-mixer
\end{tabular} 
& \xmark & \xmark \\
\midrule
ComiRec, Re4 & fixed & max pooling \\ 
\midrule
EDISON (Ours) & adaptive & \begin{tabular}[c]{@{}c@{}} max-pooling + \\ average-pooling \end{tabular} \\ \bottomrule
\end{tabular}
\caption{Comparison of various session-based recommendation models and our proposed model, focusing on the main differences.}\label{tab:framework}
\end{table}

\iffalse

\begin{table}[] \small
\begin{tabular}{c|c|c}
\toprule
Model & \begin{tabular}[c]{@{}c@{}}Multiple\\ session vectors\end{tabular} & Aggregator \\ \midrule
\begin{tabular}[c]{@{}c@{}}
GRU4Rec~\cite{HidasiKBT15GRU4Rec, HidasiK18GRU4Rec+}, NARM~\cite{LiRCRLM17NARM}, \\ 
SASRec~\cite{KangM18SASRec}, SR-GNN~\cite{WuT0WXT19SRGNN}, \\ 
NISER+~\cite{GuptaGMVS19NISER}, SGNN-HN~\cite{PanCCCR20SGNNHN},\\ 
LESSR~\cite{ChenW20LESSR}, CL4SRec~\cite{XieSLWGZDC22CL4SRec}, \\ 
CORE~\cite{hou2022core}, Atten-mixer~\cite{ZhangGLXKZXWK23Atten-Mixer}
\end{tabular} 
& \xmark & \xmark \\
% \end{tabular} & \multirow{4}{*}{\xmark} & \multirow{4}{*}{\xmark} \\
% SR-GNN~\cite{WuT0WXT19SRGNN} & \cmark & \xmark & \xmark \\
% LESSR~\cite{ChenW20LESSR} & \cmark & \xmark & \xmark \\
% NISER+~\cite{GuptaGMVS19NISER} & \cmark & \xmark & \xmark \\
% SGNN-HN~\cite{PanCCCR20SGNNHN} & \cmark & \xmark & \xmark \\
% SASRec~\cite{KangM18SASRec} & \cmark & \xmark & \xmark \\
% CL4SRec~\cite{XieSLWGZDC22CL4SRec} & \cmark & \xmark & \xmark \\
% CORE~\cite{hou2022core} & \cmark & \xmark & \xmark \\
% A-mixer~\cite{ZhangGLXKZXWK23Atten-Mixer} & \cmark & \xmark & \xmark \\
\midrule
% ComiRec~\cite{ChenZZXX21ComiRec} & \cmark & Fixed & Max pool \\
ComiRec~\cite{ChenZZXX21ComiRec}, Re4~\cite{ZhangYYLFZC022Re4} & fixed & max pooling \\ 
\midrule
% EDISON(Ours) & + $\mathbf{v}_{\text{mean}}$ & Adaptive & Max+Avg pool \\ \bottomrule
% EDISON (Ours) & Adaptive & \begin{tabular}[c]{@{}c@{}} Max-pooling + \\ Average-pooling \end{tabular} \\ \bottomrule
EDISON (Ours) & \begin{tabular}[c]{@{}c@{}} adaptive by \\ session length \end{tabular} & \begin{tabular}[c]{@{}c@{}} max-pooling + \\ average-pooling \end{tabular} \\ \bottomrule
\end{tabular}
\caption{Comparison of various session-based recommendation models and our proposed model, focusing on the main differences.}\label{tab:framework}
\end{table}

\fi

==> Tables/tab_optimal_hyperparameters.tex <==
\begin{table}[]
\centering
\begin{tabular}{c|ccccc}
\toprule
Dataset & $\tau$ & $\delta_{tr}$ & $\delta_{emb}$ & $\alpha$ & $\beta$ \\ \midrule
Dginetica & 0.07 & 0.1 & 0.1 & 1.5 & 0.9 \\
Retailrocket & 0.07 & 0.1 & 0.1 & 1.5 & 0.8 \\
Yoochoose & 0.07 & 0.1 & 0.1 & 1.5 & 0.7 \\
Tmall & 0.05 & 0.1 & 0.1 & 1.5 & 0.5 \\
Dressipi & 0.07 & 0.1 & 0.1 & 1.5 & 0.9 \\
LastFM & 0.07 & 0.1 & 0.1 & 1.5 & 0.8 \\
\bottomrule
\end{tabular}
\caption{Optimal hyperparameters of EDISON for each dataset.}\label{tab:optimal_hyper}
\end{table}

==> sec-model_backup.tex <==

\section{Proposed Model}\label{sec:framework}


\input{Figures_tex/Fig_model_architecture.tex}
In this section, we propose a novel SBR model, \emph{Multi-intent-aware Session-based Recommendation Model (\textbf{MIASRec})}, as shown in Figure~\ref{fig:architecture}. 
Our model aims to address the limitations of current SBR models in capturing multiple interests: (i) how to exhaustively represent multiple user intents inherent in each
session and (ii) how to prune out improperly represented user intent.

% Our model aims to address the limitations of current SBR models in capturing multiple interests by implementing two key components: the \emph{adaptive multi-interest extractor} and the \emph{two-sided multi-interest aggregator}. 
% (i) The adaptive extractor encodes a session and extracts multiple session vectors representing various user interests. To effectively capture the intricate user behavior, MIASRec represents multiple user interests focusing on each session item and extracts an appropriate number of session vectors based on their importance. (ii) The two-sided aggregator decodes each session vector into item distributions independently and aggregates them as the final item distribution. By employing two different pooling methods, MIASRec fully reflects the complex information contained in each session vector. In this way, MIASRec effectively extracts and aggregates multiple interests without requiring a large number of parameters.
% Lastly, we discuss MIASRec as a generalized model for existing models with either a single or multiple session vector and highlight the main differences with others.
%  focusing on each session item to accommodate complex and diverse user interests.
% The multi-interest encoder-decoder of MIASRec is capable of handling multiple session vectors. 
% Since each session item implies the user's interest at each time step, MIASRec can effectively capture the intricacies of user behaviors.

\subsection{Session-based Recommendation}\label{sec:problem_statement}
Let $\mathcal{V} = \{v_1, \dots, v_m\}$ denote a set of $m$ unique items, \eg, products and songs. An arbitrary session $s = (v_{t_1}, \dots, v_{t_{|s|}})$ represents a sequence of $|s|$ items that a user interacts with, \eg, clicks, views, and purchases. Here, $t_i$ indicates the index of the item consumed by the user at position $i$ in the session. Given a session, the goal of SBR is to predict the next item(s) that the user is most likely to consume. Formally, the SBR model takes a session as input and returns a top-$N$ item list to recommend. 


% Let $\mathcal{S} = \{s^{(1)}, \dots, s^{(n)}\}$ be a set of sessions, where $n$ is the number of sessions. An arbitrary session $s = (s_1, \dots, s_{|s|})$ represents a sequence of $|s|$ items that a user interacts with, \eg, clicks, views, and purchases. Here, $s_i \in \mathcal{V}$ indicates the $i$-th item in the session consumed by the user. Given a session, the goal of SBR is to predict the next item(s) that the user is most likely to consume. Formally, the SBR model takes a session as input and returns a top-$N$ item list to recommend. 

% \subsection{Adaptive Multi-interest Extractor}\label{sec:encoder}
\subsection{Model Architecture}\label{sec:encoder}

We first embed items as item vectors, and then apply a transformer encoder over these item embedding vectors, yielding contextualized session representations. To ensure that contextualized representations are distinct from each other and better reflect the interest associated with each session item, we adopt highway networks. 

% Then, MIASRec extracts multiple session vectors, representing various user interests. 
% \begin{equation}\label{eq:multi-encoder}
% \mathbf{h}_{1}, \dots, \mathbf{h}_{k} = \text{Extractor}(\text{Encoder}([\mathbf{v}_{1}, \dots, \mathbf{v}_{|s|}])),
% \end{equation}
% \noindent
% where $k$ denotes the adaptive number of session vectors. 
% and we introduce a mean item vector $\mathbf{v}_{\text{mean}} = \frac{1}{|s|}\sum_{i=1}^{|s|} \mathbf{v}_{i}$ reflecting a consistent user interest over session $s$. Note that $\mathbf{v}_{\text{mean}}$ depends on items in $s$.

The session encoder utilizes the bi-directional transformer encoder~\cite{VaswaniSPUJGKP17Transformer} to effectively capture the complex relationships and dependencies among items. To enhance the representation of these items, we incorporate absolute positional embedding vectors to differentiate the positions of each item. This results in the generation of multiple contextualized vectors for each item through the transformer encoder $\text{Trm}(\cdot)$ as follows:
\begin{equation}
\label{eq:transformer_output}
% \mathbf{o}_{1}, \dots, \mathbf{o}_{|s|}, \mathbf{o}_{\text{mean}} = \text{Trm}([\mathbf{v}_{1}, \dots, \mathbf{v}_{|s|}, \mathbf{v}_{\text{mean}}]).
\mathbf{o}_{1}, \dots, \mathbf{o}_{|s|} = \text{Trm}([\mathbf{v}_{1}, \dots, \mathbf{v}_{|s|}]).
\end{equation}

To ensure that each contextualized item vector better reflects the interest associated with that item and to prevent them from being similar to each other, we leverage highway networks as used in ~\cite{PanCCCR20SGNNHN}. 
\begin{equation}
\label{eq:highway}
\begin{split}
\mathbf{c}_{i} = \mathbf{g} \odot  \mathbf{v}_{i} + (1-\mathbf{g}) & \odot \mathbf{o}_{i} \ \text{for} \ i \in \{1, \dots, |s|\},  \\
 \text{where} \ \mathbf{g} =  \sigma( & \mathbf{W_{g}}[\mathbf{v}_{i};\mathbf{o}_{i}]^{\top}),
\end{split}
\end{equation}

\noindent
$\mathbf{W_{g}} \in \mathbb{R}^{d \times 2d}$ is a learnable weight matrix, $\mathbf{g} \in \mathbb{R}^{d}$ is a gating vector, $\sigma$ is the sigmoid function. 


Instead of the conventional method of utilizing a single session vector built around the last item vector, we use multiple session vectors by exploiting the potential of each item within a session. To adaptively extract user interest depending on the session, we employ a sparse transformation $\alpha$-entmax~\cite{PetersNM19entmax}. 
\begin{equation}
\alpha\text{-entmax}(\mathbf{z}) = \argmax_{ \mathbf{p} \in \Delta^{d}}{ \mathbf{p}^{\top} \mathbf{z}+H^{T}_{\alpha}(\mathbf{p})}
\end{equation}
where, $H^{T}_{\alpha}( \mathbf{p})=\frac{1}{\alpha(\alpha-1)}\sum_{j}( \mathbf{p}_j - \mathbf{p}_{j}^{\alpha})$ if $\alpha \neq 1$, else $H^{T}_{1}(p)=-\sum_{j} \mathbf{p}_j \log \mathbf{p}_j$. Depending on $\alpha$, 1-entmax and 2-entmax are equivalent to softmax and sparsemax~\cite{MartinsA16sparsemax}, respectively. When using a larger $\alpha$ value, it produces a more sparse probability distribution, and empirically, we set $\alpha$ as 1.5. We extract multiple user interests by masking contextualized item vectors.
\begin{equation}
\begin{split}
\label{eq:extractor}
\mathbf{\gamma} & = \alpha\text{-entmax}(\mathbf{w} \cdot [\mathbf{c}_{1}; \dots; \mathbf{c}_{|s|}]^{\top}),  \\
\{ \mathbf{h}_{1}, \dots, \mathbf{h}_{k} \} & = \{ \mathbf{\gamma}_{i} \mathbf{c}_{i} | \mathbf{\gamma}_{i} > 0, i \in \{1 \dots |s|\} \},
% \mathbf{j}_{1}, \dots, \mathbf{j}_{k} & = \text{argTopk}_{j \in \{1,\dots,|s|\}}(\beta), \\
% \mathbf{h}_{i} & = \mathbf{c}_{{j}_{i}} \ \text{for} \ i \in \{1, \dots, k\},
\end{split}
\end{equation}
where $\mathbf{w} \in \mathbb{R}^{d}$ is a learnable parameter and $\mathbf{\gamma} \in \mathbb{R}^{|s|}$ is importance weight vector for each item. $k$ is the number of non-zero elements in $\gamma$. Unlike previous multiple session vector models~\cite{ZhangYYLFZC022Re4, ChenZZXX21ComiRec}, our extractor adaptively determines the number of multiple session vectors for a given session.

% \subsection{Two-sided Multi-interest Aggregator}\label{sec:decoder}

% Because existing SBR models mostly employ a single session vector, it is easy to decode the session vector to an item distribution. Meanwhile, 
It is non-trivial to decode multiple session vectors to a single distribution. The decoding process of MIASRec consists of two parts: (i) decoding item distributions from each session vector representing different interests, and (ii) aggregating the distributions for the final recommendation while preserving various user interests through two pooling functions. 
% Notably, instead of selecting or aggregating multiple vectors to a single session vector, the late aggregation benefits from preserving multiple user interests.
% and preventing unnecessary intervention among session vectors at the encoder.
% \begin{equation}
% \label{eq:decoder_all}
% \mathbf{\hat{y}} = \text{Aggregator}(\text{Decoder}([\mathbf{h}_{1}, \dots, \mathbf{h}_{k}])),
% \end{equation}

First, we explain how to decode a session vector into an item distribution. As commonly used in existing studies~\cite{KangM18SASRec, hou2022core}, we employ cosine similarity, \ie, dot product with L2-normalization, to calculate item recommendation scores. Since we reuse the item embedding look-up table, the number of model parameters does not increase.  
\begin{equation}
\label{eq:decoder}
\mathbf{\hat{y}}_{1}, \dots, \mathbf{\hat{y}}_{k} = [\mathbf{\Tilde{h}}_{1}\mathbf{\Tilde{V}}^{\top}, \dots, \mathbf{\Tilde{h}}_{k}\mathbf{\Tilde{V}}^{\top}],
\end{equation}

\noindent
where $\mathbf{\Tilde{h}}_{i}$ and $\mathbf{\Tilde{V}}$ are L2-normalized session vector and normalized embedding look-up table, respectively. $\mathbf{\hat{y}}_{i} \in \mathbb{R}^m$ represents an item distribution decoded by a session vector $\mathbf{h}_{i}$. Therefore, the $j$-th element of $\mathbf{\hat{y}}_{i}$ is equal to $cos(\mathbf{h}_{i}, \mathbf{v}_{j})$.


The key challenge is how to aggregate multiple item distributions. To resolve this issue, we adopt a two-sided aggregator utilizing a combination of max-pooling and average-pooling functions without using additional parameters. Although it is possible to introduce an attention layer to calculate the significance of sessions, learning meaningful attention weights is non-trivial, \eg, the existing SBR method tends to depend on the last session vector~\cite{YuanSSWZ21DSAN}. 
\begin{equation}
\label{eq:maxpool}
\mathbf{\hat{y}} = \beta \text{MaxPool}(\mathbf{\hat{y}}_{1}, \dots, \mathbf{\hat{y}}_{k}) + (1-\beta)  \text{AvgPool}(\mathbf{\hat{y}}_{1}, \dots, \mathbf{\hat{y}}_{k}),
\end{equation}
\noindent
where $\mathbf{\hat{y}} \in \mathbb{R}^m$ is a final item distribution aggregated by multiple item distributions and $\beta$ is a combination hyperparameter. $\text{MaxPool}(\cdot)$ and $\text{AvgPool}(\cdot)$ represent the max-pooling and average-pooling functions that fetch the maximum (or average) value for each dimension from multiple vectors. Max-pooling maintains the items that reflect the principal features for multiple user interests, and average-pooling captures consistent user interest over the session. It is effective for controlling the significance of diverse user interests, helping improve the overall performance of MIASRec.


Lastly, we formulate a cross-entropy loss function between ground truth and prediction to train MIASRec.
\begin{equation}
\label{eq:recommendation_loss}
    % \mathcal{L} = - \sum^{m}_{j=1} \mathbf{y}_j\log(\mathbf{\hat{y}}_j),
    L(\mathbf{y},\mathbf{\hat{y}}) = - \sum^{m}_{j=1} \mathbf{y}(j)\log(\frac{\text{exp}(\mathbf{\hat{y}}(j) / \tau)}{\sum_i{\text{exp}(\mathbf{\hat{y}}(i) / \tau)}}),
\end{equation}
\noindent
where $\mathbf{y} \in \mathbb{R}^{m}$ is a one-hot vector of the target item, \ie, $\mathbf{y}(j)=1$ if the $j$-th item is the target item of the given session; otherwise, $\mathbf{y}(j)=0$. Here, $\tau$ is a hyperparameter to control the temperature~\cite{HintonVD15distillation} for better convergence~\cite{GuptaGMVS19NISER}. 
% MIASRec leverages max-pooling to retain the most salient user intent. However, it needs to be improved in capturing consistent user intent over the session. We thus adopt a regularization term to adjust the difference between ground truth and the average item distribution. It is effective for controlling the significance of diverse user intents, helping improve the overall performance of MIASRec.
% \begin{equation}
% \label{eq:final_loss}
%     \mathcal{L} = L(\mathbf{y},\mathbf{\hat{y}}) + \lambda \cdot L(\mathbf{y},\mathbf{\hat{y}}_{\text{avg}})
% \end{equation}

% \noindent
% where $\mathbf{\hat{y}}_{\text{avg}} = \text{AveragePool}(\mathbf{\hat{y}}_{1}, \dots, \mathbf{\hat{y}}_{k})$ is item distribution using the mean-pooling function, and $\lambda$ is a hyperparameter to adjust the weight of the regularization loss.

\iffalse
\subsection{Relationships with Other SBR Models}\label{sec:discussion}

% \input{Tables/tab_framework.tex}

% We discuss how existing models are interpreted as a specific case of MIASRec with the four key modules: a session encoder, an extractor, an item decoder, and an aggregator. 
We lastly discuss how existing models are interpreted as a specific case of MIASRec, and clarify the key differences between the proposed model and the other models.

 %in Table~\ref{tab:framework}


\vspace{2mm}
\noindent
\textbf{Single session vector representation.} Most existing models exploit neural-based encoders and represent a single session vector using a linear or an attention-based extractor. Since only a single session vector is given, the aggregator is not utilized here. Thus, the decoder directly obtains an item distribution, \ie, $\mathbf{\hat{y}_s} = \text{Decoder}(\mathbf{h}_{s})$.


First, GRU4Rec~\cite{HidasiKBT15GRU4Rec, HidasiK18GRU4Rec+} and SASRec~\cite{KangM18SASRec} adopt a GRU-based and transformer-based encoder, respectively. The extractor here selects the hidden vector of the last item as a session vector.
\begin{equation}
% \text{GRU4Rec}: \mathbf{h}_s = \text{Extractor}(\text{GRU}([\mathbf{v}_1, \ldots, \mathbf{v}_{|s|}])).
\mathbf{h}_s = \text{Extractor}(\text{GRU}([\mathbf{v}_1, \ldots, \mathbf{v}_{|s|}])).
\end{equation}
\begin{equation}
\mathbf{h}_s = \text{Extractor}(\text{Trm}([\mathbf{v}_1, \ldots, \mathbf{v}_{|s|}])).
\end{equation}

Next, SR-GNN~\cite{WuT0WXT19SRGNN} and NISER+~\cite{GuptaGMVS19NISER} utilize GNN-based encoders $\text{GNN}(\cdot)$, and the attention-based extractor $\text{Att}(\cdot)$ is used for combining multiple item vectors for a long-term preference vector which is finally combined with the last item vector $\mathbf{e}_{|s|}$ to represent a session vector. 
% two session vectors for short- and 
\begin{equation}
\begin{split}
 % \text{SR-GNN}: \mathbf{h}_s = \text{Linear}(\text{Att}(&\text{GNN}[\mathbf{v}_1,…,\mathbf{v}_{|s|}]), \mathbf{v}_{\text{mean}}), \\ 
 % \text{where} \ \ \mathbf{e}_{\text{mean}} &= \frac{1}{|s|}\sum_{i=1}^{|s|}\mathbf{v}_i
\mathbf{h}_s =  [\text{Att}([&\mathbf{c}_1,…,\mathbf{c}_{|s|}]); \mathbf{c}_{|s|}], \\ 
 \text{where} \ \ \mathbf{c}_1,…,\mathbf{c}_{|s|} &= \text{GNN}([\mathbf{v}_1,…,\mathbf{v}_{|s|}]).
\end{split}
\end{equation}

CORE~\cite{hou2022core} obtains a session vector as a weighted sum of item embedding vectors, where the DNN-based extractor $\text{DNN}(\cdot)$, such as a transformer, is used to compute the weight for each item.
\begin{equation}
\begin{split}
\mathbf{h}_s = \sum_{i=1}^{|s|} & \alpha_i \mathbf{v}_i, \\ 
 \text{where} \ \alpha_1, \dots, \alpha_{|s|} &= \text{DNN}([\mathbf{v}_1, \dots, \mathbf{v}_{|s|}]).
 % \text{where} \ \alpha_1, \dots, \alpha_{|s|} &= \text{Linear}(\text{Trm}([\mathbf{v}_1, \dots, \mathbf{v}_{|s|}]))
\end{split}
\end{equation}
% \begin{equation}
% \text{CORE}: \mathbf{h}_s = \sum_{i=1}^{|s|} \alpha_i \mathbf{e}_i \ \text{where} \ \alpha_1, \dots, \alpha_{|s|} = \text{Linear}(\text{Trm}([\mathbf{e}_1, \dots, \mathbf{e}_{|s|}]))
% \end{equation}

Although they attempt to improve session encoders or extractors, it is insufficient to represent complex and diverse user interests as a single session vector. To address this problem, MIASRec leverages multiple session vectors.

% For multiple item distributions, the late aggregator chooses candidate items for recommendation. 

\vspace{2mm}
\noindent
\textbf{Multiple session vector representation.} Within the domain of sequential recommendation for targeting long-term user histories, several models have proposed to adopt multiple vectors for handling various interests. 

ComiRec~\cite{ChenZZXX21ComiRec} and Re4~\cite{ZhangYYLFZC022Re4} represent $k$ user vectors using a weighted sum of item embedding vectors, where $k$ is defined in prior. They utilize a self-attentive extractor with trainable parameters $\mathbf{W}_1 \in \mathbb{R}^{d \times d}$ and $\mathbf{W}_2 \in \mathbb{R}^{k \times d}$. 
\begin{equation}
\label{eq:comirec}
\begin{split}
 \mathbf{h}_t &= \sum_{i=1}^{|s|}  \textbf{A}_{t,i} \mathbf{v}_i \ \text{for} \ t \in \{1, \dots, k\}, \\ 
 \text{where} \ \textbf{A} &= \text{softmax}(\mathbf{W}_2 \cdot \text{tanh}(\mathbf{W}_1\mathbf{V}_s^{\top})).
\end{split}
\end{equation}
\noindent
The sequence matrix $\mathbf{V}_s \in \mathbb{R}^{|s| \times d}=\{\textbf{v}_i\}_{i=1,\dots,|s|}$. This approach to capturing user interests is inappropriate because it assumes a fixed number of user interests, but the number of interests varies in each session. Therefore, in long sessions, they do not reflect the dynamic nature of user interests, and in short sessions, they produce redundant representations that may be noise. In contrast, MIASRec offers a more flexible approach that leverages top-$k$ (all if the session is shorter than $k$) contextualized item vectors as multiple session vectors to effectively capture complex and diverse user interests. The decoding process is similar to MIASRec, but they only utilize max-pooling to aggregate multiple vectors, ignoring the global information across multiple interests.

\fi

==> sec-preliminaries.tex <==
\section{Background}\label{sec:preliminaries}


\noindent
\textbf{Problem statement.} 
Let $\mathcal{V} = \{v_1, \dots, v_m\}$ denote a set of $m$ unique items, \eg, products and songs. Let $\mathcal{S} = \{s^{(1)}, \dots, s^{(n)}\}$ be a set of sessions, where $n$ is the number of sessions. An arbitrary session $s = (s_1, \dots, s_{|s|})$ represents a sequence of $|s|$ items that a user interacts with, \eg, clicks, views, and purchases. Here, $s_i \in \mathcal{V}$ indicates the $i$-th item in the session consumed by the user. Given a session, the goal of SBR is to predict the next item(s) that the user is most likely to consume. Formally, the SBR model takes a session as input and returns a top-$N$ item list to recommend. 




\noindent
\textbf{Key challenges.} 
To improve the accuracy of SBR, there are two main challenges to be addressed: (i) how to effectively encode a session to capture user preferences, and (ii) how to account for multiple user interests hidden in the session. Existing studies mainly focus on the former issue using neural-based session encoders such as RNNs, GNNs, and Transformers and have proven to be effective in capturing intricate relationships between items. However, these neural encoders have limitations, as they encode a single session vector to represent a session, making it difficult to capture dynamic and diverse user interests. It is particularly crucial when the session is long. 


\noindent
\textbf{Pilot study.} 
Figure~\ref{fig:exp_session_length} depicts the performance of existing SBR models~\cite{ChenZZXX21ComiRec, ZhangYYLFZC022Re4, hou2022core, GuptaGMVS19NISER, KangM18SASRec} over different session lengths. As the session length increases, the user's interest becomes more diverse and multifaceted, which leads to significant performance degradation of existing models. This problem arises from the inability of a single session representation to account for the complex and diverse nature of user interest. By using multiple representations, our proposed model achieves up to 22.6\% gains over SASRec~\cite{KangM18SASRec} for long sessions with length $\geq$ 10. Meanwhile, ComiRec~\cite{ChenZZXX21ComiRec} and Re4~\cite{ZhangYYLFZC022Re4} also utilize multiple representations, but show lower accuracy than the proposed model, indicating the importance of how well extract and aggregate multiple user interests. (Refer to Section~\ref{sec:results} for a more detailed analysis.)


\iffalse
\noindent
\textbf{Conventional framework for SBR.} 
Existing SBR models are typically built upon an encoder-decoder architecture. First, each item in the session is converted to an embedding vector using an embedding look-up table $\mathbf{V} \in \mathbb{R}^{m \times d}$, \ie, $\mathbf{v}_i = \text{Embed}(s_i) \in \mathbb{R}^d$. Here, $\mathbf{v}_{i}$ is the embedding vector of the $i$-th item in the session. Then, a session encoder represents a session as a session vector $\mathbf{h}_s$ = $\text{Encoder}([\mathbf{v}_{1}, \dots, \mathbf{v}_{|s|}]) \in \mathbb{R}^d$. Given a session vector $\mathbf{h}_s$, the decoder computes the recommendation scores for each item $v_j \in \mathcal{V}$, \ie, $\mathbf{\hat{y}} = 
\text{Decoder}(\mathbf{h}_s)$, where $\mathbf{\hat{y}} \in \mathbb{R}^{m}$. Existing studies~\cite{WuT0WXT19SRGNN, GuptaGMVS19NISER} utilize weight tying, \ie, the item embedding matrix is shared for both the encoder and the decoder. In addition, simple functions, \eg, inner product and cosine, are widely used to measure the similarity between session and item vectors for computing recommendation scores.
\fi


==> sec-relatedwork.tex <==
\section{Related Work}


% \input{Tables/tab_framework.tex}


\subsection{Session-based Recommendation}

Owing to the success of DNNs, many session-based recommenders have utilized neural-based encoders, such as RNN-, GNN-, and Transformer-based models. As the RNN-based models, GRU4Rec~\cite{HidasiKBT15GRU4Rec, HidasiK18GRU4Rec+} utilized the GRU for SBR, and NARM~\cite{LiRCRLM17NARM} improved GRU4Rec by considering both long-term and short-term preferences. RepeatNet~\cite{RenCLR0R19RepeatNet} inferred the probability of the repeated items in the session. CSRM~\cite{WangRMCMR19CSRM} combined collaborative signals between sessions using the neighbors of sessions. 

In recent studies, GNNs have been popularly used for SBR, where each session is represented by a small graph of items. SR-GNN~\cite{WuT0WXT19SRGNN} employed gated graph neural networks to capture multi-hop transitions among the session items, and NISER+~\cite{GuptaGMVS19NISER} mitigated the popularity bias and convergence issues through L2 normalization of embeddings. Besides, GCE-GNN~\cite{WangWCLMQ20GCEGNN}, MTD~\cite{HuangCXXDCBZH21MTD}, and MGIR~\cite{HanZCLSL22MGIR} handled inter-session relationships by utilizing the item transition in the global graph from whole sessions. SGNN-HN~\cite{PanCCCR20SGNNHN} summarized a session into a single vector by adopting a star node. LESSR~\cite{ChenW20LESSR} additionally used GRU to reduce multi-hop information loss in GNN. S2-DHCN~\cite{0013YYWC021S2-DHCN} and COTREC~\cite{0013YYSC21COTREC} utilized an additional supervised learning task to improve model training.
% remove redundant GNN propagation and 

Thanks to the powerful representation capacity for sequential data, transformers have been widely adopted for recommendation tasks. One of the early works in this field is SASRec~\cite{KangM18SASRec}, which utilized a transformer-based encoder and took the last contextualized hidden vector as a session vector. Subsequently, CoSAN~\cite{LuoZLZWXFS20CoSAN} improved upon SASRec~\cite{KangM18SASRec} by leveraging neighborhood sessions. To infer the user interest more elaborately, DSAN~\cite{YuanSSWZ21DSAN} attempted to learn target embedding to imitate the next target item, and ProxySR~\cite{ChoKHY21ProxySR} additionally modeled a proxy vector to infer the user's long-term preference. CL4SRec~\cite{XieSLWGZDC22CL4SRec} adopted contrastive learning to train a session encoder more effectively. Most recently, CORE~\cite{hou2022core} unified the representation space of session embeddings and item embeddings. Most existing models focus on improving neural-based encoders to express a single session vector more effectively. However, we claim that extracting and aggregating multiple user interests is crucial, especially for long and complex sessions.

%, as it helps understand and provide personalized recommendations.
% Unlike GNN-based SBR models, transformer-based models can further capture long-term dependency among items in the session. 

\subsection{Multi-interest Sequential Recommendation}
Recently, some sequential recommendation models have attempted to capture multiple user interests. MCPRN~\cite{Wang0WSOC19MCPRN} employed purpose-specific recurrent units to extract multiple purposes within a session. SINE~\cite{TanZYLZYH21SINE} leveraged a large concept pool to infer a small number of user interests. It benefits representing complex relationships in successive items. Atten-mixer~\cite{ZhangGLXKZXWK23Atten-Mixer} performs multi-level reasoning over attention mixture networks. Also, several methods~\cite{ZhuCLYYX20KA-MemNN, Chen0ZSW22Satori, LiWZMCZ22ISRec} utilized additional information, \eg, user profiles, item titles, and categories, to identify multiple user intentions. Although these methods extract multiple interest vectors from the user history, they aggregate them into a single user representation, making it difficult to reflect each interest well for recommendations.

To effectively incorporate multiple interests into recommendations, some studies have used the approach of late aggregation rather than aggregating hidden representation vectors. MIND~\cite{LiLWXZHKCLL19MIND} used dynamic capsule routing for multiple interests by clustering user history. ComiRec~\cite{ChenZZXX21ComiRec} utilized multi-head self-attention to extract different user interests. Besides, Re4~\cite{ZhangYYLFZC022Re4} builds upon ComiRec~\cite{ChenZZXX21ComiRec} by incorporating three additional backward flows for learning the multiple user interests effectively. MSGIFSR~\cite{Guo0SZWBZ22MSGIFSR} adopted consecutive item units for representing different item-level granularity using GNNs. However, because they assume a fixed number of user interests, handling dynamic and diverse user interests in sessions is difficult. While some studies~\cite{WestonWY13, PalEZZRL20Pinnersage} have also explored the representation of multiple user vectors, they do not consider the sequential/temporal order.

%at all, and therefore we do not discuss them in detail. 
% Notably, they utilize all the previous user history, making it hard to handle anonymous users in SBR.
% For aggregating multiple interests, they have difficulty in considering session consistency since they only consider the important parts of each interest through max-pooling.

\iffalse
\noindent
\textbf{Non-neural-based methods.} Without neural-based encoders, conventional solutions are classified into four directions: Markov chains (MC), rule-based, nearest-neighbors-based, and item-to-item models. First, MC~\cite{0095301MC} utilized the short-term dependency between consecutive session items. FPMC~\cite{RendleFS10FPMC} and FOSSIL~\cite{HeM16Fossil} combined MC with matrix factorization and the item-to-item model, respectively. Second, as rule-based methods, AR~\cite{AgrawalIS93AR} and SR~\cite{KamehkhoshJL17SR} utilized the item similarity from the co-occurrence between items. Third, SKNN~\cite{JannachL17SKNN} first adopted the nearest-neighbor idea for SBR, and STAN~\cite{GargGMVS19STAN} improved SKNN~\cite{JannachL17SKNN} by using sequential and temporal weights to reflect the characteristics of sessions. Lastly, item-to-item models have recently been proposed for SBR. SLIST~\cite{ChoiKLSL21SLIST} and S-Walk~\cite{ChoiKLSL22S-Walk} learn the item-to-item matrix for item correlations and transitions within sessions. Despite their simplicity, item-to-item models show comparable performance with neural-based SBR models.
% As the rule-based method, AR~\cite{AgrawalIS93AR} and SR~\cite{KamehkhoshJL17SR} utilized the item similarity from the co-occurrence between items. 
% As the rule-based method, AR~\cite{AgrawalIS93AR} utilized the item similarity from the co-occurrence between items, and SR~\cite{KamehkhoshJL17SR} improved it by considering sequential information. Although they are good at capturing short-term item dependency, they do not consider various patterns between items. They have demonstrated competitive performance, but their ability to capture high-order dependency among session items is constrained. 
\fi

==> sec-setup.tex <==
\section{Experimental Setup}\label{sec:setup}

\input{Tables/tab_data_statistics}

\input{Tables/tab_overall_performance.tex}



\textbf{Datasets.} We conduct extensive experiments on six datasets collected from e-commerce and music streaming services: Diginetica\footnote{https://competitions.codalab.org/competitions/11161}, Retailrocket\footnote{https://www.kaggle.com/retailrocket/ecommerce-dataset}, Yoochoose\footnote{https://www.kaggle.com/chadgostopp/recsys-challenge-2015}, Tmall\footnote{https://tianchi.aliyun.com/dataset/dataDetail?dataId=42}, Dressipi\footnote{https://dressipi.com/downloads/recsys-datasets/}, and LastFM\footnote{http://ocelma.net/MusicRecommendationDataset/lastfm-1K.html}. Note that the Tmall dataset is not a session dataset since it consists of long-term user shopping histories for six months. (There are timestamps in units of days, not in minutes or seconds.) However, it has been widely used in previous studies~\cite{hou2022core, LudewigJ18Evaluation, 0013YYSC21COTREC, HanZCLSL22MGIR}. Therefore, we also use it for our evaluation.
% 

For data pre-processing, we follow the conventional procedure~\cite{LudewigJ18Evaluation, LudewigMLJ19bEmpiricalAnalysis, LiRCRLM17NARM, WuT0WXT19SRGNN}. We discard the sessions with a single item and the items that occur less than five times in entire sessions. We split training, validation, and test sets chronologically as the 8:1:1 ratio. Table~\ref{tab:dataset} summarizes detailed statistics on all benchmark datasets.

\noindent
\textbf{Baselines.} We compare MIASRec with the following SBR models. \textbf{SASRec}~\cite{KangM18SASRec} use a transformer-based encoder. \textbf{SR-GNN}~\cite{WuT0WXT19SRGNN} uses a GNN-based encoder to capture multi-hop item relationships in the session. \textbf{NISER+}~\cite{GuptaGMVS19NISER} improves SR-GNN through L2 normalization of item embedding vectors. \textbf{SGNN-HN}~\cite{PanCCCR20SGNNHN} adopts a star node and a highway network to capture two-hop correlations among items effectively. \textbf{DSAN}~\cite{YuanSSWZ21DSAN} apply sparse transformation function to denoise the irrelevant session items using learned target item embedding. \textbf{CORE}~\cite{hou2022core} is a state-of-the-art model representing sessions and items on a consistent embedding space.
% \textbf{LESSR}~\cite{ChenW20LESSR} utilizes GNN and transformer to encode a session vector.

We also compare with the subsequent multi-interest models. \textbf{SINE}~\cite{TanZYLZYH21SINE} extracts multi-interest embeddings from a large concept pool and aggregates as a user embedding vector. \textbf{Atten-mixer(A-mixer)}~\cite{ZhangGLXKZXWK23} leverages multi-level attention mixture network to achieve multi-level reasoning over item transitions. \textbf{ComiRec}~\cite{ChenZZXX21ComiRec} employ self-attention mechanism to learn multi-interest representation. \textbf{Re4}~\cite{ZhangYYLFZC022Re4} improves ComiRec by leveraging backward flows for interest embedding learning.

Note that we do not compare ours with SBR models using additional information, such as temporal information~\cite{gng-ode, TMIGNN} or content-based features~\cite{HidasiQKT16p-RNN} for a fair comparison. All experimental results were averaged over three runs with different seeds, and we conducted the significance test using a paired t-test. 
% For more details about implementation and hyperparameter settings, please refer to Appendix~\ref{sec:app_implementation}.
% one RNN-based model~\cite{LiRCRLM17NARM}. NARM~\cite{LiRCRLM17NARM} employs an attention-based GRU-based encoder to improve GRU4Rec~\cite{HidasiK18GRU4Rec+}.



\noindent
\textbf{Evaluation protocol and metrics}. As the common protocol to evaluate SBR models~\cite{LiRCRLM17NARM, WuT0WXT19SRGNN}, we adopt the \emph{iterative revealing scheme}, which iteratively exposes an item from a session to the model. For evaluation metrics, we adopt Recall (R@$N$) and Mean Reciprocal Rank (M@$N$), to quantify the prediction accuracy of the next single item. We use cutoff $N$ = \{10, 20\}, where $N$ = 20 is by default.
%  It is effective for evaluating sequential user behavior throughout an entire session. 


\noindent
\textbf{Implementation details.} For reproducibility, we implemented MIASRec and the other baseline models on an open-source recommendation system library RecBole\footnote{https://github.com/RUCAIBox/RecBole}~\cite{ZhaoMHLCPLLWTMF21RecBole, ZhaoHPYZLZBTSCX22RecBole2.0}. We optimized all the baselines using Adam optimizer ~\cite{KingmaB14Adam} with a learning rate of 0.001. We set the dimension of the embedding vectors to 100 and the max session length to 50. We stopped the training if the MRR@20 on the validation set decreased for three consecutive epochs. For all methods, we set the batch size to 1024. For MIASRec, we set $\alpha$ as 1.5 for $\alpha$-entmax and tune the temperature $\tau$ among \{0.01, 0.05, 0.07, 0.1, 0.5, 1\}, dropout ratio $\delta$ among \{0, 0.1, 0.2, 0.3, 0.4, 0.5\}. We search the combination hyperparameter $\beta$ from 0 to 1 in 0.1 increments. We followed the original papers' settings for other hyperparameters of each baseline model, but if not available, we thoroughly tuned them. We finally report the performance on the test set using the models that show the highest performance on the validation set. We conduct all experiments on a server with 2 NVidia A6000, 512 GB memory, and 2 Intel Xeon Processor E5-2695 v4 (2.10 GHz, 45M cache). 
% All source codes will be publicly available upon acceptance.
% $\lambda$ among \{0, 0.01, 0.1, 0.5, 1, 2, 5\}
% RecBole-GNN\footnote{https://github.com/RUCAIBox/RecBole-GNN}, and RecBole-TRM\footnote{https://github.com/RUCAIBox/RecBole-TRM}

% \textbf{Baseline models.} We compare MIASRec with nine SBR models, including one RNN-based model~\cite{LiRCRLM17NARM}, four GNN-based models~\cite{WuT0WXT19SRGNN, GuptaGMVS19NISER, PanCCCR20SGNNHN, ChenW20LESSR}, and four transformer-based models~\cite{KangM18SASRec, XuZLSXZFZ19GCSAN, XieSLWGZDC22CL4SRec, hou2022core}. Specifically, NARM~\cite{LiRCRLM17NARM} employs an attention-based GRU-based encoder to improve GRU4Rec~\cite{HidasiK18GRU4Rec+}. SR-GNN~\cite{WuT0WXT19SRGNN} uses a GNN-based encoder to capture multi-hop item relationships in the session. NISER+~\cite{GuptaGMVS19NISER} improves SR-GNN~\cite{WuT0WXT19SRGNN} through L2 normalization for item embedding vectors. SGNN-HN~\cite{PanCCCR20SGNNHN} adopts a star node and a high-way network to capture two-hop correlations among items effectively. LESSR~\cite{ChenW20LESSR} utilizes the GNN and transformer to encode a session vector. Meanwhile, SASRec~\cite{KangM18SASRec}, GC-SAN~\cite{XuZLSXZFZ19GCSAN}, and CL4SRec~\cite{XieSLWGZDC22CL4SRec} uses a transformer-based encoder for SBR. GC-SAN~\cite{XuZLSXZFZ19GCSAN} utilizes neighbor sessions to leverage collaborative information, and CL4SRec~\cite{XieSLWGZDC22CL4SRec} introduces a contrastive loss to learn better session representations. CORE~\cite{hou2022core} is a state-of-the-art transformer-based model representing sessions and items on a consistent embedding space. Note that we do not compare ours with SBR models using additional information, such as temporal information~\cite{gng-ode, TMIGNN} or content-based features~\cite{HidasiQKT16p-RNN} for a fair comparison. We also do not compare ours with multi-interest sequential recommender models~\cite{ChenZZXX21ComiRec, ZhangYYLFZC022Re4} because they are mainly designed to capture long-term multi-interest preferences from all the previous user histories. All experimental results were averaged over five runs with different random seeds, and we conducted the significance test using a paired t-test at $\rho$ < 0.05. For more details about implementation and hyperparameter settings, please refer to Appendix~\ref{sec:app_implementation}.

